EgoAdapt: A multi-stream evaluation study of adaptation to real-world egocentric user video

In egocentric action recognition a single population model is typically trained and subsequently embodied on a head-mounted device, such as an augmented reality headset. While this model remains static for new users and environments, we introduce an adaptive paradigm of two phases, where after pretraining a population model, the model adapts on-device and online to the user's experience. This setting is highly challenging due to the change from population to user domain and the distribution shifts in the user's data stream. Coping with the latter in-stream distribution shifts is the focus of continual learning, where progress has been rooted in controlled benchmarks but challenges faced in real-world applications often remain unaddressed. We introduce EgoAdapt, a benchmark for real-world egocentric action recognition that facilitates our two-phased adaptive paradigm, and real-world challenges naturally occur in the egocentric video streams from Ego4d, such as long-tailed action distributions and large-scale classification over 2740 actions. We introduce an evaluation framework that directly exploits the user's data stream with new metrics to measure the adaptation gain over the population model, online generalization, and hindsight performance. In contrast to single-stream evaluation in existing works, our framework proposes a meta-evaluation that aggregates the results from 50 independent user streams. We provide an extensive empirical study for finetuning and experience replay.

==> additional_data.tex <==






==> backup.tex <==
















-------------------- OLD INTRO BELOW



One of the cornerstones to improving human-computer interaction is for machine-learning systems to understand or predict human behavior~\cite{HCIintelligent}.
A head-mounted device, such as an augmented reality headset, enables a first-person viewpoint from the user, 
where recognizing the user's actions is key to building such improved understanding.
Current egocentric action recognition models aim for generalization to new users through training on videos from a vast and diverse population of users~\cite{Feichtenhofer_2019_ICCV,Fan_2021_ICCV}.
However, this population model remains unchanged on the user device, disregarding factors that are highly prone to change over time such as user behavior and preferences, and the surrounding environment.
The distribution shift from population model to user, and the non-stationarity over the user's experiences are highly challenging, given neural networks are prone to \emph{catastrophic forgetting} of previous knowledge~\cite{french1999catastrophic}.
Although overcoming this forgetting is the main focus of \emph{continual learning}, 
existing benchmarks are often artificially created from static datasets~\cite{lopez2017gradient,aljundi2019online,De_Lange_2021_ICCV,chrysakis20a}, focus on adapting to a single stream~\cite{Wang_2021_ICCV,lin2021clear,cai2021online}, and are non-existing for egocentric action recognition.
Therefore, we propose the egocentric action recognition benchmark \textbf{EgoAdapt}, addressing both the distribution shift from population to user, and adapting to the user's experience in an online fashion in the real world.
To this end, EgoAdapt entails video from Ego4d~\cite{ego4d} for 50 real-world egocentric user streams instead of a single stream, and spans 53 different scenarios with 2740 unique actions over 77 hours of annotated video. 
We evaluate performance fully online and completely task-agnostic, and introduce \emph{Adaptation Gain} metrics to directly measure the model's improvement over the population model.
Furthermore, we conduct an extensive empirical study on the novel user-adaptation setup in EgoAdapt, scrutinizing the learning dynamics of online finetuning and standard continual learning method Experience Replay (ER)~\cite{chaudhry2019continual,Verwimp_2021_ICCV}.
We find that personalization offers significant improvements over the population model even with simple online finetuning, while adapting the features or revisiting samples with ER greatly ameliorates forgetting without losing online generalization performance.
Our transfer study between user models indicates the models become true experts of the user stream, with significant improvement over the population model, but trading off generalization to other user streams.
\looseness=-1






